Imitation Bootstrapped Reinforcement Learning

Despite the considerable potential of reinforcement learning (RL), robotic control tasks predominantly rely on imitation learning (IL) due to its better sample efficiency. However, it is costly to collect comprehensive expert demonstrations that enable IL to generalize to all possible scenarios, and any distribution shift would require recollecting data for finetuning. Therefore, RL is appealing if it can build upon IL as an efficient autonomous self-improvement procedure. We propose imitation bootstrapped reinforcement learning (IBRL), a novel framework for sample-efficient RL with demonstrations that first trains an IL policy on the provided demonstrations and then uses it to propose alternative actions for both online exploration and bootstrapping target values. Compared to prior works that oversample the demonstrations or regularize RL with an additional imitation loss, IBRL is able to utilize high quality actions from IL policies since the beginning of training, which greatly accelerates exploration and training efficiency. We evaluate IBRL on 6 simulation and 3 real-world tasks spanning various difficulty levels. IBRL significantly outperforms prior methods and the improvement is particularly more prominent in harder tasks.

==> sections/10_rebuttal.tex <==
\begin{center}
\noindent\textbf{Rebuttal for ``Imitation Bootstrapped Reinforcement Learning", Paper-ID 374}
\end{center}

\noindent\textbf{Overall Response}

We appreciate the valuable feedback from the reviewers and we are delighted that the reviewers find this work \emph{``a novel approach"}, \emph{``does a good job of selecting appropriate baselines and ablations"}, \emph{``simple, elegant, modular"}. We have conducted additional experiments and discussions to address the reviewer's comments. 
To briefly summarize the new contents and the corresponding problems that they address:
\begin{itemize}
    \item \textbf{Meta Reviewer:} More implementation details on RLPD and RFT in Appendix \cref{app:impl}.
    \item \textbf{Reviewer RA7B:} Actor dropout in Meta-World in Appendix \cref{app:actor-dropout-mw}. Meta-World is too simple to differentiate between the different methods once they reach certain level of performance and sample efficiency. IBRL and RFT perform similarly with and without actor dropout in Meta-World.
    \item \textbf{Reviewer k1rw, 5LcH:} The role and impact of IL policy in IBRL in Appendix \cref{app:il-in-ibrl}. We show the percentage of actions from the IL policy during training. We also run IBRL with an imitation policy trained from suboptimal data and show that IBRL can eventually escape from such suboptimal IL policy.
    \item \textbf{Reviewer 5LcH:} Comparison with Residual Policy Learning (RPL) in Appendix \cref{app:rpl}. IBRL performs noticeably better than RPL. We also find that IBRL can be combined with RPL to further improve performance.
    \item \textbf{Reviewer k1rw, Meta Reviewer:} Comparison with Regularized Optimal Transport (ROT), an inverse RL/online imitation learning method, in Appendix \cref{app:rot}. IBRL performs significantly better (95\% success rate vs 30\% after same amount online interaction) than ROT which does not use the sparse reward from the environment.
\end{itemize}

Please see the the following pages for individual response to each reviewer.
\begin{itemize}
    \item \hyperlink{page.2}{Meta Reviewer -- Page 2}
    \item \hyperlink{page.3}{Reviewer RA7B -- page 3,4}
    \item \hyperlink{page.5}{Reviewer k1rw -- page 5,6}
    \item \hyperlink{page.7}{Reviewer 5LcH -- page 7}
\end{itemize}


\newpage
\begin{center}
\noindent\textbf{Response to Meta Reviewer}
\end{center}

\noindent We appreciate the constructive feedback from you as well as other reviewers.

\noindent\textbf{More Details on Baselines, RFT vs. ROT:}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{It would also be useful to clearly state what SOTA algorithms are being used in the case of RLPD and RFT. \\Is RFT just Regularized Optimal Transport?
}
\end{tcolorbox}

In the paper, we mention that RFT and RLPD use the same TD3 backbone as IBRL. They also share the same techniques that are commonly used in state-of-the-art RL implementations such as Q-ensemble (i.e., RED-Q, for states), image augmentation (DrQ v2, for images) and network designs (layer normalization, etc.). The RFT baseline is essentially ROT without the OT dense reward but instead using the environment sparse 0/1 reward. When the sparse reward is available, we find the predicted OT reward to be harmful for the performance as it makes training unstable and hard to tune the balance between ground truth sparse reward and OT dense reward. Same as RLPD and IBRL, we also add demonstrations to the replay buffer in RFT, which is not part of the original ROT method but improves performance. We have added additional implementation details on RFT and RLPD in Appendix~\cref{app:impl} and quote it here for easy access. 

\begin{tcolorbox}[colback=gray!10,boxrule=0pt,colframe=white]
The RLPD and RFT baselines share the same base RL implementation as IBRL. The core idea of RLPD~\cite{ball2023efficient} is to draw half of the batch from demonstrations and the other half from the RL replay buffer to upweigh the successful demonstration trajectories to address the exploration challenge. Note that the original RLPD paper use SAC as the base RL algorithm while our implementation use the same TD3 as IBRL for controlled experiments. Note that the original RLPD disables the entropy backup part of SAC in 3 out of 4 benchmarks evaluated, making that specific SAC variant highly similar to TD3 in practice. 

RFT first pretrains the encoder and policy head with BC and then runs RL with an additional BC loss term on the policy head for regularization. Different instantiations of this idea have appeared in prior works~\cite{nair2018overcoming}. Specifically, our implementation of RFT resembles the one from ROT~\cite{haldar2022watch-rot}. The policy loss is
$L_\theta(\pi_{\theta}) = -E_{s \sim \mathcal{D}}Q(s, \pi_\theta(s)) + \alpha \lambda(\pi_\theta) E_{(s, a)\sim \mathcal{T}} \| a - \pi_\theta(s) \|^2 $, where $\mathcal{D}$ is the RL replay buffer and $\mathcal{T}$ is the demonstration dataset. Moreover, $\alpha$ is the base regularization weight and we set $\lambda(\pi_\theta) = E_{s\sim \mathcal{T}} [\mathbbm{1}_{Q(s, \pi^0_\theta(s)) > Q(s, \pi_\theta(s))}]$ to dynamically adjust the weight of regularization. $\pi^0_\theta(s)$ is the pretrained policy.
\end{tcolorbox}

Suggested by another reviewer, we also compare against the original ROT to emphasize the difference in the assumption (sparse reward vs. predicted reward) and show that IBRL performs significantly better than ROT in Appendix~\cref{app:rot}.

\noindent\textbf{Types of Regularization, Comparison to Residual Policy Learning:}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{There are questions such as the type of regularization that can be used (KL such as PPO) and comparisons to other approaches such as residual policy learning.}
\end{tcolorbox}

One of the main goals of this work is to achieve high sample efficiency. Being an on-policy method, PPO is notably less sample efficient and cannot easily train on demonstration data. Therefore, in this work, in line with many prior works focusing on sample efficiency and real world applications, we focus on off-policy Q-learning methods. The BC loss term in RFT is essentially a form of KL regularization assuming that the action distribution is isotropic Gaussian with fixed variance.

We run residual policy learning (RPL) and show that IBRL performs better than RPL (see ~\cref{fig:rpl-xyz}). We also note that RPL and IBRL are compatible and show that we can further improve sample efficiency by combining both methods. 

\noindent\textbf{Addressing Other Reviewers Comments:}
% We have also addressed reviewers' individual concerns in their respective responses. To summarize:

\emph{Reviewer RA7B} is mainly concerned about the similar performance between IBRL and RFT on the Meta-World tasks and ask for more ablations on actor dropout on Meta-World. We argue that Meta-World is the simplest setting evaluated in this paper and they are mainly a sanity check. We list details on why Meta-World is simple and arguably too simple to differentiate strong methods such as IBRL and (well tuned) RFT. We also show results of IBRL, RFT and RPLD on Meta-World with actor dropout enabled.

\emph{Reviewer k1rw} would like to know if IBRL sacrifices any exploration coverage and suggests using an imitation policy not well aligned with the goal. 
We run IBRL with significantly worse BC policies (50\% worse) and show that IBRL can escape from the proposals of such BC and eventually converge to similar optimal final performance at a slower speed. 
We show the frequency of the IL action being selected during the course of RL training per reviewer's request. We also compare to ROT following their request on adding an inverse RL baseline.

\emph{Reviewer 5LcH} is interested in residual policy learning (RPL) as an additional baseline as well as frequency of the IL action being selected. We include new plots to address both of them.

\newpage
\begin{center}
\noindent\textbf{Response to Reviewer RA7B}
\end{center}

\noindent Thank you for your constructive feedback. Please allow us to address your concerns here.

\noindent \textbf{Performance of IBRL and RFT on Meta-World}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{... Method outperforms in some domains and only matches the performance in others.  ... This could suggest hyperparameter tuning or other issues are limiting the performance of the baselines.}
\end{tcolorbox}

This is in fact because the tasks are too simple to differentiate between the efficacy and strength of the methods. Specifically, Meta-World is simple because of smaller action space (4 dimension vs. 7 dimension in Robomimic and real robot) and shorter episode length (45 in Meta-World Assembly vs. 150 in Robomimic Square), and significantly less randomness in the initial conditions. Its simplicity is also reflected in the number of samples required for convergence. We use the hard tasks from the Meta-World suite but still they only require 20K-40K samples for IBRL and RFT to solve. In comparison, the two Robomimic tasks require 100K and 500K samples, and are much closer to more challenging real-world environments we’d be interested in. Due to its simplicity, it is not surprising that Meta-World is unsuitable for differentiating between the methods, and we use it mostly because it was used as a baseline for prior work and can be thought of as a way to sanity check the performance of different techniques. 

Note that we have carefully tuned the regularization weight for RFT and show the \emph{best} one in the paper. 
So the fact that IBRL matches the \emph{best} of RFT emphasizes the advantage of IBRL as it requires no extra hyperparameters or tuning to balance RL and IL. 
We have implemented many of the bells and whistles that improve sample efficiency for both RFT and RLPD. 
Note that our implementation of RFT is $20\%$ better and RLPD is $10\%$ better than MoDem, a model-based approach published in 2023 that outperforms a wide range of methods on this Meta-World benchmark.

~

\noindent \textbf{Actor Dropout in Meta-World:}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{What do the plots for Meta-World look like with Actor Dropout for all applicable baselines?}
\end{tcolorbox}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/metaworld_dropout.pdf}
\caption{Performance of RFT with actor dropout compared with IBRL counterparts. Actor dropout does not meaningfully change the performance of these strong methods on the relatively simple Meta-World benchmark.}
\label{fig:metaworld-dropout1-xyz}
\vspace{-2mm}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/metaworld_dropout2.pdf}
\caption{Performance of RLPD with actor dropout compared with IBRL counterparts. Actor dropout slightly improves RLPD.}
\label{fig:metaworld-dropout2-xyz}
\vspace{-4mm}
\end{figure}

\cref{fig:metaworld-dropout1-xyz} and \cref{fig:metaworld-dropout2-xyz} compare the performance of IBRL, RFT and RLPD with and without actor dropout enabled on Meta-World. The inclusion of actor dropout does not make a notable difference for IBRL and RFT, while slightly improves RLPD. We have not tried actor dropout in MoDem because it is a vastly different algorithm and uses completely different architectures.
For the same reason stated above, we argue that Meta-World is not a good environment to differentiate methods once they reach certain levels of sample efficiency. Therefore the similar performance is not a negative sign of either IBRL nor actor dropout.
We add these plots to Appendix~\cref{app:actor-dropout-mw} and quote the corresponding discussion here for the ease of reading. 


\begin{tcolorbox}[colback=gray!10,boxrule=0pt,colframe=white]
In the main paper, we do not include actor dropout in all methods on Meta-World as it does not meaningfully affect the conclusion in this simple benchmark. \cref{fig:metaworld-dropout1} and \cref{fig:metaworld-dropout2} shows the performance of IBRL, RFT and RLPD with and without actor dropout. Actor dropout slightly improves RLPD but makes little difference for IBRL and RFT which are already highly competitive in this benchmark.

Given these results, we want to emphasize that Meta-World is a relatively simple benchmark for single task RL as it is originally proposed for meta-learning and thus the designers ensure that each individual task can be solved easily~\cite{yu2019meta-world}. Specifically, Meta-World has smaller actions space (4 dimensional instead of 7 dimensional in Robomimic and real world), shorter episode length (less than 100 steps) and limited randomness in the initial condition. In the sparse reward setting considered in this paper, we observe that Meta-World tasks are easy for modern RL methods that utilize demonstrations even under highly limited data (i.e., 3 episodes of demonstrations). Therefore, these tasks do not provide enough signal to differentiate strong methods like IBRL and RFT, nor to justify the benefit of regularization techniques like actor dropout.
\end{tcolorbox}


\noindent \textbf{Is IBRL better solely because of actor dropout?}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{IBRL uses dropout but baseline approaches are not evaluated with dropout by default. When dropout is added baseline performance improves significantly. It’s therefore not clear whether IBRL is superior because it uses the BC data better or because it simply uses a better optimization technique.}
\end{tcolorbox}

The ablation in \cref{fig:actor_dropout} and \cref{fig:ibrl_ablation} show that 1) even with actor dropout, the performance of baselines do not exceed IBRL, and 2) actor proposal, bootstrap proposal, and actor dropout all play an important role to the strong performance of IBRL. 

Additionally, although dropout is a widely used technique, to the best of our knowledge, it is not a well known fact that dropout in the \emph{actor} significantly improves sample efficiency in RL for continuous control. The closest prior work studies dropout in the \emph{critic} [1] and only applies it in state-based RL. Therefore, we consider actor dropout one of the architectural innovations and a contribution of our work supported by the strong performance of \emph{RFT + Actor dropout} as shown in \cref{fig:actor_dropout}.

~

\noindent [1] Hiraoka et al. Dropout Q-Functions for Doubly Efficient Reinforcement Learning



\newpage
\begin{center}
\noindent\textbf{Response to Reviewer k1rw}
\end{center}

\noindent Thank you for your insightful feedback and suggestions. We have added plots and experiments to address your questions!

\noindent\textbf{Suboptimal IL Policy:}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{\textbf{Theoretical implication:} ... The algorithm appears to work in practice, but is probably giving up the possibility of exploring the entire state space in service of acceptable performance. A neat experimental evaluation of this would be to use an imitator policy that is trained on high quality demonstrations that are not aligned to optimize the true reward for the policy at hand. ...}
\\

\emph{What would happen if the demonstrations were misaligned with the true sparse reward the task was optimizing for. Would the RL policy be able to recover from that?
}
\end{tcolorbox}

\begin{figure}[h]
\centering
\includegraphics[width=0.5\linewidth]{figs/mh_ibrl.pdf}
\caption{IBRL with a significantly worse BC policy trained from suboptimal demonstrations. This illustrates that IBRL can escape from substantially worse BC policies and achieve similar final performance at the cost of lower initial performance.}
\label{fig:worse-bc-xyz}
\vspace{-2mm}
\end{figure}

Thanks for the suggestion. We interpret the question as whether IBRL can still recover an ``optimal" solution if the imitation policy is suboptimal due to misaligned data or other reasons. We train suboptimal imitation policy using lower quality demonstrations from the Multi-Human (MH) version of the Robomimic dataset instead of the Proficient-Human (PH) version used in normal IBRL. The episodes in the MH dataset are noisier and inefficient, making the learned BC policy significantly worse. The average length of the 50 demonstrations in the MH dataset is 271  compared to 149 in the PH dataset.
We then use this worse BC policy in IBRL and show the results in ~\cref{fig:worse-bc-xyz}. We see that \emph{BC (worse)} is roughly $50\%$ worse than the original BC trained on a Proficient-Human dataset and it does have some negative impact to the sample efficiency of IBRL. However, IBRL with worse BC is able to eventually converge to a similar final performance as IBRL with normal BC, essentially \emph{escaping} from the suboptimality of the BC. We add the plot and a new paragraph in Appendix~\cref{app:il-in-ibrl}.

\noindent\textbf{Selection of IL Action Proposals:}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{Would it be possible to add plots that indicate the rate at which imitation policy actions vs RL policy actions were chosen as a function of epochs trained on.}
\end{tcolorbox}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/action_selection.pdf}
\caption{Percentage of actions from the IL policy selected during IBRL training.}
\label{fig:action-selection-xyz2}
\vspace{-2mm}
\end{figure}

\cref{fig:action-selection-xyz2} shows the rate at which imitation policy actions vs RL policy actions were chosen. IBRL selects a decent amount of actions from the imitation policy throughout the training. The rate of selecting imitation policy actions first increases (as the critic gets better) and then decreases (as the RL policy gets better). We add this plot the more discuss in Appendix \cref{app:il-in-ibrl} and quote it here.

\begin{tcolorbox}[colback=gray!10,boxrule=0pt,colframe=white]
To understand the role of the IL policy during IBRL training and at convergence, in \cref{fig:action-selection-xyz2} we plot the frequency that IBRL selects the IL action when collecting online data for training. IBRL selects fewer actions from the IL policy at the beginning, because the critics are randomly initialized and it is easy for the RL actor to find actions with ``fake" high Q-values. As the critics get updated, the incorrectly high Q-values for those actions are pushed down and IBRL starts to pick more actions from IL policy as the critic learns that those IL actions are high quality by learning from the demonstration data in the replay buffer. Then, the ratio of IL actions steadily decreases in most cases as the RL policy improves. One exception is in the hardest real world Hang task, where the ratio of IL actions keeps increasing.
This is reasonable given that the IL policy is fairly strong for this task and the RL policy likely has not fully converged yet, as reflected by the high performance of IL and imperfect performance of IBRL in this task. In all cases, however, the ratio never decreases to zero, indicating that IBRL still relies on the IL policies, which are parameterized by much deeper networks, even at convergence.
\end{tcolorbox}

\noindent\textbf{Comparison to ROT Baseline:}

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{\textbf{Broader baseline selection:} I would have appreciated including other ways of incorporating demonstration data as a part of baselines (IRL for example) as a way of developing intuition about how the proposed method differs in peak performance from radically different approaches.}
\end{tcolorbox}


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/rot.pdf}
\caption{Comparison with IBRL and ROT, one of the best performing RL method that does not require environment reward. Note IBRL and ROT have \textbf{different assumptions} because ROT does not use the sparse 0/1 reward from the environment. This comparison is mainly to illustrate the difference in the peak performance under different assumptions (sparse reward v.s. no environment reward at all).}
\label{fig:rot-xyz}
\end{figure}


We add comparisons to regularized optimal transport (ROT), one of the strongest online imitation/inverse RL methods, a family of methods that do not rely on environment reward. \cref{fig:rot-xyz} shows the results. We highlight that the peak performance of IBRL, which assumes access to environment sparse reward, is significantly higher than ROT which only uses predicted dense reward from optimal transport (OT). We have more discussion in Appendix \cref{app:rot} and again quote it here.

\begin{tcolorbox}[colback=gray!10,boxrule=0pt,colframe=white]

To understand the difference in the peak performance between RL with sparse reward and RL that assumes no access to environment reward at all (such as inverse RL, or online imitation learning), we compare IBRL against ROT~\cite{haldar2022watch-rot}, a powerful online imitation learning method that has shown to outperform a wide range of other inverse RL methods. Our RFT baseline is closely related to ROT. ROT can be seen as RFT without the sparse reward from the environment but instead with a dense trajectory matching reward computed by optimal transport. We emphasize the methods considered in this paper have \textbf{different assumptions} from ROT or inverse RL/online imitation in general as the later family of methods do no assume access of any environment rewards and instead use reward predicted from demonstrations.
\\

~\cref{fig:rot} shows IBRL and ROT on the Meta-World tasks. Unsurprisingly, IBRL performs significantly better than ROT. Note that the Meta-World tasks considered in this paper are harder than the ones considered in the original ROT paper and we also run on significantly smaller sample budgets (60K vs 1M). Additionally, we find that adding OT reward on IBRL or RFT no longer helps but sometimes hurts performance when having access to the ground truth sparse reward as it is challenging to balance the magnitude of the two reward sources.
\end{tcolorbox}

\newpage
\begin{center}
\noindent\textbf{Response to Reviewer 5LcH}
\end{center}


\noindent Thank you for your valuable comments. We address your questions below.

\noindent\textbf{Comparison to Residual Policy Learning:} 

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{I am curious how does this method compare to approaches like Residual Policy Learning?}
\end{tcolorbox}

The suggestion of residual policy learning (RPL) is a great idea. We implement RPL using the same BC policy as IBRL for the base policy and we use RL to train a residual policy whose last layer is initialized to zero following the RPL paper. 
As shown in \cref{fig:rpl-xyz}, RPL achieves slightly better performance than RLPD and RFT but still underperforms IBRL. 
We also note that RPL and IBRL are fully compatible and so we implement IBRL with the residual policy framework and find that the resulting IBRL-RPL further improves the performance over IBRL.

\begin{figure}[h]
\centering
\includegraphics[width=0.55\linewidth]{figs/rpl.pdf}
\vspace{-2mm}
\caption{Performance of Residual Policy Learning (RPL) compared with IBRL and other baselines. RPL uses the same ResNet-18 BC policy as the base policy. RPL performs well among the baselines but still underperforms IBRL. We can incorporate RPL formulation for the policy network into IBRL and the resulted IBRL-RPL gains some extra improvement on top of IBRL.}
\label{fig:rpl-xyz}
\vspace{-2mm}
\end{figure}

We add a new~\cref{app:rpl} in Appendix to discuss RPL and IBRL-RPL. For ease of reading, we quote the section here.

\begin{tcolorbox}[colback=gray!10,boxrule=0pt,colframe=white]
In this section, we compare IBRL with an additional baseline, residual policy learning (RPL)~\cite{rpl}. The core concept of residual policy learning is to first have a base policy $\mu(s)$ and then use RL to learn a policy $\pi(s)$ that outputs action residual to the first policy. The final action from RPL takes the form of $a = \mu(s) + \pi(s)$. Our instantiation of RPL uses the same deep ResNet-18 BC policies as IBRL and we also allow the RL residual policy to take the output of the BC policy as an additional input to provide it with a useful initial guess, i.e. $a = \mu(s) + \pi(s, \mu(s))$. The BC policy is kept fixed and we optimize the residual policy using the same RL backbone used by all model-free RL methods in this paper. Furthermore, we follow~\cite{rpl} to zero out the last layer of the RL policy in RPL so that the initial actions are close to the BC actions. 

\cref{fig:rpl-xyz} shows the performance of RPL alongside IBRL and other baselines in the two Robomimic tasks with image inputs. RPL performs well compared against other baselines but not as well as IBRL. Inspired by the strong performance of RPL, we are interested in understanding if the residual formulation benefits other methods. Therefore, we additionally run IBRL with an RPL-style modification to the input and output of the policy network (IBRL-RPL, dotted line in~\cref{fig:rpl-xyz}). We find that IBRL-RPL further improves the sample efficiency over IBRL on the harder Square task and maintains roughly the same performance on the simpler Can task. It is encouraging that IBRL can be combined with existing techniques to achieve even better performance.
\end{tcolorbox}


\noindent\textbf{Selection of IL Action Proposals:} 

We add new plots to address this feedback:

\begin{tcolorbox}[colback=pink!10,boxrule=0pt,colframe=white]
\emph{As learning converges, does the RL policy get used in all parts of the state space, or does the IL always have higher value? I would be curious to see where in the state space each policy is chosen for action selection during the learning phases.}
\end{tcolorbox}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figs/action_selection.pdf}
\caption{Percentage of actions from the IL policy selected during IBRL training.}
\label{fig:action-selection-xyz}
\vspace{-2mm}
\end{figure}

\cref{fig:action-selection-xyz} illustrate the percentage of online inference actions from IL policy during IBRL training. IBRL always picks a non-trivial amount of actions from the IL policy even after training for a long time. IBRL selects fewer actions from the IL at the beginning, because the critics are not yet well trained and it is easy for the RL actor to find suboptimal actions with high estimated Q-values. Those Q-values are then pushed down and IBRL starts to pick more actions from IL policy as the critic learns from the demonstration data that those actions are good. Then the ratio of IL actions steadily decreases in most cases as RL policy improves.
We have included this plot and discussions in \cref{app:il-in-ibrl} of Appendix. We quote it here for easy access:

\begin{tcolorbox}[colback=gray!10,boxrule=0pt,colframe=white]
To understand the role of the IL policy during IBRL training and at convergence, in \cref{fig:action-selection-xyz} we plot the frequency that IBRL selects the IL action when collecting online data for training. IBRL selects fewer actions from the IL policy at the beginning, because the critics are randomly initialized and it is easy for the RL actor to find actions with ``fake" high Q-values. As the critics get updated, the incorrectly high Q-values for those actions are pushed down and IBRL starts to pick more actions from IL policy as the critic learns that those IL actions are high quality by learning from the demonstration data in the replay buffer. Then, the ratio of IL actions steadily decreases in most cases as the RL policy improves. One exception is in the hardest real world Hang task, where the ratio of IL actions keeps increasing.
This is reasonable given that the IL policy is fairly strong for this task and the RL policy likely has not fully converged yet, as reflected by the high performance of IL and imperfect performance of IBRL in this task. In all cases, however, the ratio never decreases to zero, indicating that IBRL still relies on the IL policies, which are parameterized by much deeper networks, even at convergence.
\end{tcolorbox}




